Rank-Metric Codes and Their Applications

The rank metric measures the distance between two matrices by the rank of their difference. Codes designed for the rank metric have attracted considerable attention in recent years, reinforced by network coding and further motivated by a variety of applications. In code-based cryptography, the hardness of the corresponding generic decoding problem can lead to systems with reduced public-key size. In distributed data storage, codes in the rank metric have been used repeatedly to construct codes with locality, and in coded caching, they have been employed for the placement of coded symbols. This survey gives a general introduction to rank-metric codes, explains their most important applications, and highlights their relevance to these areas of research.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> ch_furtherApps.tex <==
\chapter{Further Applications}
\todo{
    \begin{itemize}
    \item Remove space-time codes section.
    \item Lia: Move coded caching section into storage chapter.
    \item Antonia: Write something about Private information retrieval over networks \cite{TajedineHollantiWZ-2018} (in network chapter or in conclusion)
    \item Sven: Mention "Linear authentication codes~\cite{wang2003linear}", "Space-time codes"\cite{Gabidulin2000Spacetime,Lusina2003Maximum,Lu2004Generalized,AugotLoidreauRobert-GabidulinCharacteristicZero_2013,puchinger2016space,kamche2019rank}, and "Digital image watermarking \cite{lefevre2019application}" only in the conclusion 
    \end{itemize}
}
Further applications: space-time codes, low-rank matrix recover, PIR over networks, any other application that comes to our minds (Sven, Antonia, everyone)


\newpage
\section{Space-Time Codes}

\todo{early draft, need to be improved}
Space-time codes \cite{tarokh1998space} are designed for multiple-input/multiple-output (MIMO) facing channels in point-to-point single-user (multi-antenna) scenarios.
In the literature, there are various space-time code constructions \todo{add citations, and also mention multi-block space-time codes}.

A space-time code is a set of complex matrices.
The rows of a codeword (matrix) correspond to the symbols transmitted over the same antenna, and the columns of a codeword are those symbols transmitted in the same time step---hence the name space(antenna)--time codes.
There are several design criteria for space-time codes \cite{tarokh1998space}.
One of the most important ones is that the diversity gain of the space-time coding scheme is determined by the minimum rank distance (over the complex field) of the space-time code.

This criterion motivated a line of work that started in 2000, in which codewords of a finite-field maximum rank distance code were mapped entry-wise to complex matrices using a rank-metric preserving mapping.


\subsection{Channel Model and Design Criteria}

\newcommand{\Ntx}{N_\mathrm{tx}}
\newcommand{\Nrx}{N_\mathrm{rx}}
\newcommand{\Ntime}{N_\mathrm{time}}
\newcommand{\N}{\ve{N}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\Xset}{\mathcal{X}}

We consider a flat-fading MIMO channel with additive white Gaussian noise.
We assume that the channel has $\Ntx$ transmit antennas, $\Nrx$ receive antennas, and we encode over $\Ntime$ time steps.
This means that the sent codeword is a complex matrix $\X \in \CC^{\Ntx \times \Ntime}$ and the received word is of the form $\Y \in \CC^{\Nrx \times \Ntime}$.
We have
\begin{align*}
\Y = \H \X + \N,
\end{align*}
where $\H \in \CC^{\Nrx \times \Ntx}$ is the channel matrix and its entries are chosen i.i.d.\ from the zero-mean unit-variance complex Gaussian distribution, and $\N \in \CC^{\Nrx \times \Ntx}$ is the noise matrix, whose entries are chosen i.i.d.\ from a zero-mean complex Gaussian distribution.
We assume that $\H$ is known at the receiver, but $\N$ is not known.
\todo{SNR}

A space-time code is a set of complex matrices $\Xset \subseteq \CC^{\Ntx \times \Nrx}$.
The aim of a decoder is to find
\begin{align*}
\hat{\X} = \argmin_{\X \in \Xset} \lVert \Y-\H\X \rVert_\mathsf{F},
\end{align*}
where $\lVert \cdot \rVert_\mathsf{F}$ is the Frobenius matrix norm.


\begin{itemize}
	\item Recall main design criteria by Tarokh et al.
	\item State decoding strategies
\end{itemize}


\subsection{Space-Time Code Constructions based on Rank-Metric Codes}

\todo{Add a tikz picture with an illustration of the encoding scheme}

\todo{Add a table with the schemes (codes, mappings, modulation alphabet)}

\todo{Also include multi-block space-time codes? (based on sum-rank metric)}


\subsection{Private Information Retrieval over Networks}
Privacy is a major concern for Internet or network users. Whenever a user downloads a file from a server, they reveal their interest in the requested file. Private information retrieval (PIR) allows a user to hide the identity of their requested file from the servers. PIR was first introduced in \cite{chor1998private}, where the data is assumed to be replicated on multiple servers and the user is able to retrieve the file she wants privately. It was also proved that if the data is stored on a single server, then the only way to achieve PIR in the \emph{information theoretic} sense, \emph{i.e.}, privacy with no restrictions on the computational power of the server, is to download all the files.


In \citep{TajedineHollantiWZ-2018}, the problem of providing privacy to users requesting data over a network from a distributed storage system (DSS) is considered. The DSS, which is considered as the multi-terminal destination of the network from the user's perspective, is encoded by an MRD code to store the data on these multiple servers. A private information retrieval (PIR) scheme ensures that a user can request a file without revealing any information on which file is being requested to any of the servers. In this paper, a novel PIR scheme is proposed, allowing the user to recover a file from a storage system with low communication cost, while allowing some servers in the system to collude in the quest of revealing the identity of the requested file. The network is modeled as a random linear network, \emph{i.e.}, all nodes of the network forward random (unknown) linear combinations of incoming packets. Both error-free and erroneous random linear networks are considered.

\aw{How much more details do we want?}

\subsection{Open Problems}

\todo{State that there is no proper analysis of the other design criteria, yet, and that somebody should really also compare the rank-metric-based codes with other important space-time codes in the literature w.r.t.\ these criteria and/or FER/SNR plots.}







==> main-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {main}


==> main-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {main}


==> main-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {main}


==> main-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {main}


==> main-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {main}


==> main-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {main}

